The Dawn of GUI Agent: A Preliminary Case Study with Claude 3.5 Computer Use

The recently released model, Claude 3.5 Computer Use, stands out as the first frontier AI model to offer computer use in public beta as a graphical user interface (GUI) agent. As an early beta, its capability in the real-world complex environment remains unknown. In this case study to explore Claude 3.5 Computer Use, we curate and organize a collection of carefully designed tasks spanning a variety of domains and software. Observations from these cases demonstrate Claude 3.5 Computer Use's unprecedented ability in end-to-end language to desktop actions. Along with this study, we provide an out-of-the-box agent framework for deploying API-based GUI automation models with easy implementation. Our case studies aim to showcase a groundwork of capabilities and limitations of Claude 3.5 Computer Use with detailed analyses and bring to the fore questions about planning, action, and critic, which must be considered for future improvement. We hope this preliminary exploration will inspire future research into the GUI agent community. All the test cases in the paper can be tried through the project: https://github.com/showlab/computer_use_ootb.

==> tables/abaltions.tex <==
\begin{table}[t]
\centering
\caption{Ablation studies on different tagging methods.
}
\small % 9 9
% \normalsize % 10 10
% \fontsize{8.3pt}{\baselineskip}\selectfont % font size
\renewcommand\tabcolsep{2.5pt} % column space
% \renewcommand\arraystretch{0.93} % line space
\begin{tabular}{l|c|ccccc} 
\toprule
 Model & Overall & General & Install & Apps & Single & Webshop \\
 \midrule
By side & 48.39 & 35.24 & 42.18 & 42.46 & 81.50 & 40.53\\ 
\midrule
Red & 49.05 & 41.61 & 35.00 & 43.81  & 76.50 & 48.32 \\
\midrule 
Center	&  49.72  & 47.93 & 36.06 & 44.54 & 79.50  & 40.58 \\
\bottomrule
\end{tabular}
 \label{tab:ablation_tags}
\end{table}

\begin{table}[t]
\centering
\caption{Ablation studies on different prompts.
}
\small % 9 9
% \normalsize % 10 10
% \fontsize{8.3pt}{\baselineskip}\selectfont % font size
\renewcommand\tabcolsep{2.5pt} % column space
% \renewcommand\arraystretch{0.93} % line space
\begin{tabular}{l|c|ccccc} 
\toprule
 Model & Overall & General & Install & Apps & Single & Webshop \\
 \midrule
Baseline& 48.39 & 35.24 & 42.18 & 42.46 & 81.50 & 40.53\\ 
\midrule 
Think	&  46.66  & 35.01 & 39.12 & 40.50  & 76.50 & 42.18 \\
\midrule
Specific & 48.77 & 50.77 & 40.54 & 42.32 & 69.50  & 40.71 \\
\bottomrule
\end{tabular}
 \label{tab:ablation_prompts}
\end{table}

==> tables/dataset_statistics.tex <==
\begin{table}[t]
\centering
{\small
% \vspace{-6mm}
\caption{The Android in the Wild (AITW) dataset~\citep{Rawles2023AndroidIT} statistics\label{tab:data_stats}.}
% \vspace{-6mm}
 \setlength{\tabcolsep}{2pt}
    \centering
    \begin{tabular}{lrrr}
    \toprule
     {Dataset}  & Episodes & Screens  &  Instructions\\
    \midrule
     General & 9,476 & 85,413 & 545 \\
     Install &  25,760 & 250,058 & 688 \\
     GoogleApps &  625,542 & 4,903,601 & 306  \\
     Single & 26,303 & 85,668 & 15,366 \\
     WebShopping & 28,061 & 365,253 & 13,473 \\
    \bottomrule
  \end{tabular}
  }
  \vspace{-3mm}
\end{table}

==> tables/ios.tex <==
\begin{table}[t]
\centering
{\small
% \vspace{-6mm}
\caption{Zero-shot \gptname iOS screen navigation accuracy on the ``intended action description'' and ``localized action execution'' tasks, respectively.\label{tab:iosexp}}
% \vspace{-6mm}
\setlength{\tabcolsep}{3pt}
    \begin{tabular}{lcc}
    \toprule
      Setting & \multicolumn{2}{c}{Accuracy}\\
    \midrule
     Intended Action Description & 50/55\ \ = & 90.9\%  \\
     Localized Action Execution &  41/55\ \ = & 74.5\%  \\
    \bottomrule
  \end{tabular}
  }
  % \vspace{-6mm}
\end{table}

==> tables/main_results.tex <==
\begin{table*}[t]
\centering
\caption{Main results (\%). Segment 1: fine-tuned Llama 2 baseline; Segment 2: in-context learning LLM baselines. ``ZS'' stands for ``zero-shot.''; Segment 3: GPT-4V zero-shot results: ``image-only'' means only screen images are fed into the agent. ``+text'' adds parsed screen descriptions. ``+history'' allows the agent to access its history actions.  ``Training Free'' means a model with zero-shot performance or in-context learning. ``Text Free'' means no parsed screen description is needed. The overall score is computed as the average over all the subsets.
}
\small % 9 9
% \fontsize{8.3pt}{\baselineskip}\selectfont % font size
\renewcommand\tabcolsep{3pt} % column space
% \renewcommand\arraystretch{0.93} % line space

\begin{tabular}{l|cc|c|ccccc} 
\toprule
 Model & Training Free & Text Free & Overall & General & Install & GoogleApps & Single & WebShopping \\
 \midrule
Fine-tuned Llama 2 & \ngmark & \ngmark & 28.40 & 28.56 & 35.18 & 30.99 & 27.35 & 19.92\\ 
\midrule 
PaLM 2 ZS & \okmark & \ngmark& 30.90	&  -  &  - &  - &  -  & - \\
PaLM 2 5-shot & \okmark & \ngmark& 39.60	&  -  &  - &  - &  -  & - \\
ChatGPT 5-shot & \okmark& \ngmark & 7.72 &	5.93	&4.38	&10.47	& 9.39	& 8.42\\
\midrule
\gptname ZS image-only & \okmark & \okmark & 50.54 & 41.66 & 42.64 & \textbf{49.82} & 72.83  & 45.73 \\
\gptname ZS +text & \okmark & \ngmark & 51.92 & 42.44 & \textbf{49.18} & 48.26 & 76.34 & 43.35 \\
\gptname ZS +history & \okmark & \ngmark & \textbf{52.96} & \textbf{43.01} & 46.14 & 49.18 & \textbf{78.29} & \textbf{48.18} \\
\bottomrule
\end{tabular}
 \label{tab:main_results}
\end{table*}

% \begin{table*}[t]
% \centering
% \caption{Main results (\%). Segment 1: fine-tuned Llama 2 baseline; Segment 2: in-context learning LLM baselines. ``ZS'' stands for ``zero-shot.''; Segment 3: GPT-4V zero-shot results: ``image-only'' means only screen images are fed into the agent. ``+text'' adds parsed screen descriptions. ``+history'' adds a memory module to track history.  ``Training Free'' means a model with zero-shot performance or in-context learning. ``Text Free'' means no parsed screen description is needed. The overall score is computed as the average over all the subsets.
% }
% \small % 9 9
% % \fontsize{8.3pt}{\baselineskip}\selectfont % font size
% \renewcommand\tabcolsep{3pt} % column space
% % \renewcommand\arraystretch{0.93} % line space

% \begin{tabular}{l|cc|c|ccccc} 
% \toprule
%  Model & Training Free & Text Free & Overall & General & Install & GoogleApps & Single & WebShopping \\
%  \midrule
% Fine-tuned Llama 2 & \ngmark & \ngmark & 28.40 & 28.56 & 35.18 & 30.99 & 27.35 & 19.92\\ 
% \midrule 
% PaLM 2 ZS & \okmark & \ngmark& 30.90	&  -  &  - &  - &  -  & - \\
% PaLM 2 5-shot & \okmark & \ngmark& 39.60	&  -  &  - &  - &  -  & - \\
% ChatGPT 5-shot & \okmark& \ngmark & 7.72 &	5.93	&4.38	&10.47	& 9.39	& 8.42\\
% \midrule
% % GPT-4 ZS text-only & \okmark & \ngmark & 50.01 & 38.64 & \textbf{51.26} & 46.11 & 73.21 & 40.82\\ \midrule
% \gptname ZS image-only & \okmark & \okmark & 50.54 & 41.66 & 42.64 & \textbf{49.82} & 72.83  & 45.73 \\
% \gptname ZS +text & \okmark & \ngmark & 51.92 & 42.44 & \textbf{49.18} & 48.26 & 76.34 & 43.35 \\
% \gptname ZS +history & \okmark & \ngmark & \textbf{52.96} & \textbf{43.01} & 46.14 & 49.18 & \textbf{78.29} & \textbf{48.18} \\
% % \gptname 2-shot & \okmark & \okmark & \textbf{52.61} & \textbf{46.84} & 44.67 & \textbf{50.44} & \textbf{74.41}  & \textbf{46.68} \\
% \bottomrule
% \end{tabular}
%  \label{tab:main_results}
% \end{table*}

% \begin{table*}[t]
% \centering
% \caption{Main results (\%). Segment 1: specialized agent baselines; Segment 2: in-context learning LLM baselines; Segment 3: fine-tuned Llama 2 baseline; Segment 4: GPT-4V results. Prior published best results are marked with an \underline{underline}. ``Unified'' means a general model that can work across subsets. ``w/o Anno.'' means no screen description is needed. The BC and PaLM-CoT results are from \citet{rawles2023android}. The other results are based on our own implementations. The overall score is computed as the average accuracy on all the subsets.
% The best average result is in \textbf{bold} face.}

% % \scriptsize % 7 7
% % \footnotesize % 8 8
% \small % 9 9
% % \normalsize % 10 10
% % \fontsize{8.3pt}{\baselineskip}\selectfont % font size
% \renewcommand\tabcolsep{3pt} % column space
% % \renewcommand\arraystretch{0.93} % line space

% \begin{tabular}{l|cc|c|ccccc} 
% \toprule
%  Model & No Training & w/o Anno. & Overall & General & Install & GoogleApps & Single & WebShopping \\
%  \midrule
% BC-single & \ngmark & \ngmark & 68.7	& - & - &  - &  -  &\\
% BC-history & \ngmark & \ngmark& \underline{73.1} &	\underline{63.7}	& \underline{77.5}	& \underline{75.7}	& \underline{80.3}	& \underline{68.5} \\
% \midrule
% Auto-UI$_\text{separate}$ & \ngmark & \okmark & 74.07 & 65.94 & \textbf{77.62} & \textbf{76.45} & 81.39 & 69.72 \\
% Auto-UI$_\text{unified}$ & \ngmark & \okmark & \textbf{74.27}	& \textbf{68.24} &	{76.89} & {71.37} & \textbf{84.58} & \textbf{70.26} \\
%  \midrule
% PaLM 2-ZS & \okmark & \ngmark& 30.90	&  -  &  - &  - &  -  &\\
% PaLM 2 5-shot & \okmark & \ngmark& 39.60	&  -  &  - &  - &  -  &\\
% ChatGPT 5-shot & \okmark& \ngmark &7.72 &	5.93	&4.38	&10.47	& 9.39	& 8.42\\
% \midrule
% Fine-tuned Llama 2 & \ngmark & \ngmark & 28.40 & 28.56 & 35.18 & 30.99 & 27.35 & 19.92\\ 
% \midrule 
% \gptname & \okmark & \okmark & 49.77 & 42.18 & 41.72 & 48.14 & 71.52  & 45.27 \\
% \bottomrule
% \end{tabular}
%  \label{tab:main_results}
% \end{table*}
